On the Risk of Cancelable Biometrics

Cancelable biometrics (CB) employs an irreversible transformation to convert the biometric features into transformed templates while preserving the relative distance between two templates for security and privacy protection. However, distance preservation invites unexpected security issues such as pre-image attacks, which are often neglected.This paper presents a generalized pre-image attack method and its extension version that operates on practical CB systems. We theoretically reveal that distance preservation property is a vulnerability source in the CB schemes. We then propose an empirical information leakage estimation algorithm to access the pre-image attack risk of the CB schemes. The experiments conducted with six CB schemes designed for the face, iris and fingerprint, demonstrate that the risks originating from the distance computed from two transformed templates significantly compromise the security of CB schemes. Our work reveals the potential risk of existing CB systems theoretically and experimentally.

==> PR/old.tex <==

% \section{Feasibility of the attack on cancelable biometrics\label{section.attacktheory}}
% \subsection{Linear transformation}
% For the sake of simplicity, we firstly analyze the situation of linear projection based approaches, such as random projection. The transformation function in such kind of cancelable biometrics can be generalized to a matrix projection, i.e., $y=x W$. Let us consider (\ref{eq.objectivefinal}) with $n=1$. The loss function, based on the 2-norm distance, can be expressed as
% \begin{equation}
% l=\lVert \hat{\bm{x}}\bm{W_C} - \bm{y_0}\lVert=\lVert \hat{\bm{x}}\bm{W_C} - \bm{x_0W_C}\lVert, \label{eq.feasibility.lossfun}
% \end{equation}
% where $W_{C}$ represents the projection matrix in $Sys~C$, $\bm{y_0}$ is the compromised template known by the attacker, and $\hat{\bm{x}}$ is the pre-image to be resonstructed.
% In order to explain how the intrinsic nature of the biometric features and the projection matrix may influence the rate of successful attacks, the following proposition has been formulated.

% \begin{prop}
% Given a compromised template $\bm{x_0W_C}$, a new biometric feature vector $\bm{x_1}$, where both $\bm{x_1}$ and $\bm{x_0}$ belong to same person, and another projection matrix $\bm{W_T}$ from $Sys~T$, assume that:

% (i) Algorithm \ref{algo.SimilaritybasedAttackGA} is convergent;

% (ii) $\lVert \bm{W_*}\lVert \leq M $ where $M$ is a constant;

% (iii) $\bm{x_1} = \bm{x_0} + \bm{\delta} $ where $\bm{\delta}$ is the random noise among biometric feature vectors from the same person;

% (iv) Value  
% \begin{equation}
% \epsilon \triangleq max \lVert \hat{\bm{x}}\bm{W_C} - \bm{x_0W_C}\lVert \label{eq.feasibility.funmax}
% \end{equation}
% is bounded.

% Given the output $\hat{\bm{x}}$ of Algorithm \ref{algo.SimilaritybasedAttackGA}, then:

% (i) $\lVert \hat{\bm{x}}\bm{W_C} - \bm{x_1W_C}\lVert$ has an upper bound which is the sum of $\epsilon$ and $M\lVert \bm{\delta}\lVert$;

% (ii)  $\lVert \hat{\bm{x}}\bm{W_T} - \bm{x_1W_T}\lVert$ has an upper bound which is linear in $\epsilon$.
% \end{prop}

% \begin{proof}
% From Eq. (\ref{eq.feasibility.funmax}), we have $\lVert \hat{\bm{x}}\bm{W_C} - \bm{x_0W_C}\lVert < \epsilon$, thus, 
% \begin{equation}
% \begin{split}
% \lVert \hat{\bm{x}}\bm{W_C} - \bm{x_1W_C}\lVert & = \lVert \hat{\bm{x}}\bm{W_C} - (\bm{x_0}+\bm{\delta})\bm{W_C}\lVert = \lVert (\hat{\bm{x}}\bm{W_C} - \bm{x_0}\bm{W_C})-\bm{\delta}\bm{W_C}\lVert \\
% & \leq \epsilon +\lVert \bm{\delta}\bm{W_C}\lVert \\
% & \leq \epsilon +M\lVert \bm{\delta}\lVert ,
% \end{split}
%  \label{eq.feasibility.stscupperbound}
% \end{equation}
% which provides an upper bound $\epsilon$ with an additional residual $M\lVert \bm{\delta}\lVert$.

% Next, an auxiliary projection matrix $\bm{W_\Delta}$ is introduced, based on the natural characteristics of projection operation, to represent $\bm{W_T} = \bm{W_C}\bm{W_\Delta}$. Intuitively, $\bm{W_\Delta}$ can be regarded as an alternative projection to project the vector in $Sys~C$ into $Sys~T$. In other words, $\bm{W_T}$ and $\bm{W_C}\bm{W_\Delta}$ perform the same projection. Thus,
% \begin{equation}
% \begin{split}
% \lVert \hat{\bm{x}}\bm{W_T} - \bm{x_1W_T}\lVert & = \lVert \hat{\bm{x}}\bm{W_T} - (\bm{x_0}+\bm{\delta})\bm{W_T}\lVert = \lVert \hat{\bm{x}}\bm{W_C}\bm{W_\Delta} - \bm{x_0}\bm{W_C}\bm{W_\Delta}-\bm{\delta}\bm{W_C}\bm{W_\Delta}\lVert \\
% & = \lVert ( \hat{\bm{x}}\bm{W_C} - \bm{x_0}\bm{W_C}-\bm{\delta}\bm{W_C})\bm{W_\Delta}\lVert \\
% & \leq (\epsilon +\lVert \bm{\delta}\bm{W_C}\lVert) \lVert \bm{W_\Delta} \lVert \leq M (\epsilon +\lVert \bm{\delta}\bm{W_C}\lVert) \\
% & \leq M (\epsilon+M\lVert \bm{\delta}\lVert),
% \end{split}
%  \label{eq.feasibility.stscupperbound2}
% \end{equation}
% which provides an upper bound that is linear in $\epsilon$.
% \end{proof}

% According to the proposition above, the attack can succeed as long as the attacker can achieve a low value of $\epsilon$ in a single system. For example, if the attacker compromises the template in $Sys~C$, and then uses the pre-image $\bm{\hat{x}}$ to access $Sys~C$. The feasibility of using $\bm{\hat{x}}$ to access $Sys~T$ depends on both $\epsilon$ and $M$.

% Let us consider BioHashing as a case study to illustrate the feasibility of the attack in a real scenario. While BioHashing consists of a random projection and threshold-based binarization, only the random projection, which perforns the main dimensionality reduction, will be considered. In \cite{teoh_random_2006}, a random matrix is first generated from a Gaussian distribution, then an orthogonalization is performed to generate the projection matrix of the BioHashing. Hence, for BioHashing, it is safe to conclude that $\lVert \bm{W_*}\lVert = M =1 $. Thus both $\lVert \hat{\bm{x}}\bm{W_C} - \bm{x_1W_C}\lVert$ and $\lVert \hat{\bm{x}}\bm{W_T} - \bm{x_1W_T}\lVert$ have an upper bound of $\epsilon +\lVert \bm{\delta}\lVert$. If Algorithm \ref{algo.SimilaritybasedAttackGA} can achieve a lower $\epsilon$, it is highly possible for the attacker, by exceeding the system threshold, to bypass any system regardless of $\bm{W}$.

% \subsection{Non-Linear transformation}
% While most cancellable transformations indeed is not a linear mapping between feature space and transformed template space. In this subsection we consider the situation of non-linear transform based cancelable biometrics. For simplicity, we formulate the cancelable transformation as a combination of  non-linear mapping function $\sigma(\cdot)$ and a linear projection:
% \begin{equation}
%     y=\sigma (\bm{x}\bm{W_C})
% \end{equation}
% The goal now becomes:
% \begin{equation}
% l=\lVert \sigma (\hat{\bm{x}}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C}) \lVert \label{eq.feasibility.lossfun_nonlinear}
% \end{equation}
% Same as aforementioned discussion on linear mapping, another proposition can be formulated.

% \begin{prop}
% Given a compromised template $\sigma (\bm{x}_0\bm{W_C})$, a new biometric feature vector $\bm{x_1}$, where both $\bm{x_1}$ and $\bm{x_0}$ belong to same person, and another projection matrix $\bm{W_T}$ from $Sys~T$, assume that:

% (i) Algorithm \ref{algo.SimilaritybasedAttackGA} is convergent; Hence value  
% \begin{equation}
% \epsilon \triangleq max \lVert \sigma (\hat{\bm{x}}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C})\lVert \label{eq.feasibility.funmax_nonlinear}
% \end{equation}
% is bounded.

% (ii) $\bm{x_1} = \bm{x_0} + \bm{\delta} $ where $\bm{\delta}$ is the random noise among biometric feature vectors from the same person; There exists $\omega>0$, $\lVert \sigma (\bm{x_0}W) -  \sigma (\bm{x_0}W + \bm{\delta}W) \lVert < \omega $;

% % (iii) $\sigma (\bm{x_1}W) = \sigma ((\bm{x_0} + \bm{\delta})W)= \sigma (\bm{x_0}W + \bm{\delta}W)$ where $\bm{\delta}$ is the random noise among biometric feature vectors from the same person;

% Given the output $\hat{\bm{x}}$ of Algorithm \ref{algo.SimilaritybasedAttackGA}, then:

% (i) $\lVert \sigma (\hat{\bm{x}}\bm{W_C}) - \sigma (\bm{x}_1\bm{W_C}) )\lVert$ has an upper bound which is the sum of $\epsilon$ and $M\lVert \bm{\delta}\lVert$;

% (ii)  $\lVert \sigma (\hat{\bm{x}}\bm{W_T}) - \sigma (\bm{x}_1\bm{W_T}) )\lVert$ has an upper bound which is linear in $\epsilon$.
% \end{prop}

% \begin{proof}
% From Eq. (\ref{eq.feasibility.funmax_nonlinear}), we have $\lVert \sigma (\hat{\bm{x}}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C}) )\lVert < \epsilon$, thus, 
% \begin{equation}
% \begin{split}
% \lVert \sigma (\hat{\bm{x}}\bm{W_C}）) - \sigma (\bm{x_1W_C})\lVert & = \lVert \sigma (\hat{\bm{x}}\bm{W_C}) -\sigma ( (\bm{x_0}+\bm{\delta})\bm{W_C})\lVert = \lVert (\hat{\bm{x}}\bm{W_C} - \bm{x_0}\bm{W_C})-\bm{\delta}\bm{W_C}\lVert \\
% & \leq \epsilon +\lVert \bm{\delta}\bm{W_C}\lVert \\
% & \leq \epsilon +M\lVert \bm{\delta}\lVert ,
% \end{split}
%  \label{eq.feasibility.stscupperbound_nonlinear}
% \end{equation}
% which provides an upper bound $\epsilon$ with an additional residual $M\lVert \bm{\delta}\lVert$.

% Next, an auxiliary projection matrix $\bm{W_\Delta}$ is introduced, based on the natural characteristics of projection operation, to represent $\bm{W_T} = \bm{W_C}\bm{W_\Delta}$. Intuitively, $\bm{W_\Delta}$ can be regarded as an alternative projection to project the vector in $Sys~C$ into $Sys~T$. In other words, $\bm{W_T}$ and $\bm{W_C}\bm{W_\Delta}$ perform the same projection. Thus,
% \begin{equation}
% \begin{split}
% \lVert \hat{\bm{x}}\bm{W_T} - \bm{x_1W_T}\lVert & = \lVert \hat{\bm{x}}\bm{W_T} - (\bm{x_0}+\bm{\delta})\bm{W_T}\lVert = \lVert \hat{\bm{x}}\bm{W_C}\bm{W_\Delta} - \bm{x_0}\bm{W_C}\bm{W_\Delta}-\bm{\delta}\bm{W_C}\bm{W_\Delta}\lVert \\
% & = \lVert ( \hat{\bm{x}}\bm{W_C} - \bm{x_0}\bm{W_C}-\bm{\delta}\bm{W_C})\bm{W_\Delta}\lVert \\
% & \leq (\epsilon +\lVert \bm{\delta}\bm{W_C}\lVert) \lVert \bm{W_\Delta} \lVert \leq M (\epsilon +\lVert \bm{\delta}\bm{W_C}\lVert) \\
% & \leq M (\epsilon+M\lVert \bm{\delta}\lVert),
% \end{split}
%  \label{eq.feasibility.stscupperbound2}
% \end{equation}
% which provides an upper bound that is linear in $\epsilon$.
% \end{proof}




% where $W_{C}$ represents the projection matrix in $Sys~C$, $\bm{y_0}$ is the compromised template known by the attacker, and $\hat{\bm{x}}$ is the pre-image to be resonstructed.

% \XBupdate{Here we need to discuss on linear transform and non-linear transform. Add $\sigma()$ as the non-linear mapping, keep in mind that the mapping need to preserve the distance. Finally, we will have $\lVert \sigma (\hat{\bm{x}}\bm{W_C}) - \sigma (\hat{\bm{x}_1}\bm{W_C}) )\lVert=\lVert \sigma (\bm{x}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C}+\delta\bm{W_C}) )\lVert$, and we need to assume $ \lVert \sigma (\bm{x}_0\bm{W_C}) )\lVert - \epsilon_{lo}<\lVert \sigma (\bm{x}_0\bm{W_C}+\delta\bm{W_C}) )\lVert< \lVert \sigma (\bm{x}_0\bm{W_C}) )\lVert + \epsilon_{up}$}

% \XBupdate{then, we can conclude that  $\lVert \sigma (\bm{x}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C}+\delta\bm{W_C}) )\lVert < \lVert \sigma (\bm{x}\bm{W_C}) - \sigma (\bm{x}_0\bm{W_C}) )\lVert + \epsilon <\epsilon$ }


% \subsection{Information leakage at the feature level}
% In a cancelable biometric system, the random vector $\{\bm{x_1},...,\bm{x_n}\} \in \mathcal{X}$ is the original feature vector with the corresponding protected template $\{\bm{y_1},...,\bm{y_n}\} \in \mathcal{Y}$. Even though the vectors $\bm{x_i}$ and $\bm{y_i}$ can be either composed of real or binary values, for simplicity, only binary vectors will be considered.

% By measuring the entropy, the amount of information in $\mathcal{X}$ (attacker’s initial uncertainty), the amount of information leaked to $\mathcal{Y}$, and the amount of unleaked information about $\mathcal{X}$ (attacker’s remaining uncertainty) can be computed \cite{smith2009foundations}. Firstly, the entropy of $\mathcal{X}$ can be defined as
% \begin{equation}
% H(\mathcal{X}) =-\sum_{\bm{x}\in \mathcal{X}} p(\bm{x}) \log p(\bm{x})
% \end{equation}
% The conditional entropy, measuring the uncertainty about $\mathcal{X}$ under the exposure of $\mathcal{Y}$, can be defined as
% \begin{equation}
% H(\mathcal{X}|\mathcal{Y} ) = -\sum_{\bm{y}\in \mathcal{Y}} p(\bm{y})\sum_{\bm{x}\in \mathcal{X}} p(\bm{x}|\bm{y}) \log p(\bm{x}|\bm{y}) \label{eq.conditionentropy}
% \end{equation}
% as $H(\mathcal{X}|\mathcal{Y} )=0$, $\mathcal{X}$ can be completely retrieved from $\mathcal{Y}$, and as the maximum $H(\mathcal{X}|\mathcal{Y} )=H(\mathcal{X}) $, $\mathcal{X}$ and $\mathcal{Y}$ are totally independent. 

% The mutual information between $\mathcal{X}$ and $\mathcal{Y}$, denoted by $I(\mathcal{X};\mathcal{Y})$, can be exploited to evaluate the information learned from a known $\mathcal{Y}$. Given a cancelable biometric transformation $f \in \mathcal{F}$, a protected template $\mathcal{Y}$ can be generated by $\mathcal{Y}=f(\mathcal{X})$, where $\mathcal{X}$ represents the original instance of the biometric feature vector. The mutual information is then
% \begin{equation}
% I(\mathcal{X} ; \mathcal{Y}) =H(\mathcal{X})-H(\mathcal{X} | \mathcal{Y}) \label{eq.mutual1},
% \end{equation}
% where $I(\mathcal{X};\mathcal{Y})=I(\mathcal{Y};\mathcal{X})$, and $0<I(\mathcal{X};\mathcal{Y} )<H(\mathcal{X})$. Specifically,  $I(\mathcal{X};\mathcal{Y} )=0$ means that $\mathcal{X}$ and $\mathcal{Y}$ are independent, while $I(\mathcal{X};\mathcal{Y} )=H(\mathcal{X})$ means they are totally dependent.

% In reality, the attacker could retrieve several instances of the protected template from the same person, represented by multiple instances of $\mathcal{Y}$. In order to answer the straightforward question ``Will the multiple instances $\mathcal{Y}$ help the attacker to gain more information about $\mathcal{X}$?'' the conditional mutual information is defined first:

% \begin{define}
% For random variables $A$, $B$ and $C$, the conditional mutual information is defined by 
% \begin{equation}
% I(A ; B | C) \triangleq H( A | C )-H( A |B, C). \label{eq.mutual2}
% \end{equation}
% \end{define}
% Considering the simple case where $n=2$, i.e., two instances in $\mathcal{Y}$ are compromised, it can be shown that increasing the number of compromised instances of the template also increases the attack risk. 
% \begin{coro}
% From Eqs (\ref{eq.mutual1}) and (\ref{eq.mutual2}), the mutual information $I(\mathcal{X} ; \mathcal{Y}_{1},\mathcal{Y}_{2} )$ can be computed by
% \begin{equation}
% \begin{aligned} &I(\mathcal{X} ; \mathcal{Y}_{1},\mathcal{Y}_{2} ) =H(\mathcal{X})-H(\mathcal{X} | \mathcal{Y}_{1}, \mathcal{Y}_{2}) \\ &=H(\mathcal{X})-H(\mathcal{X} | \mathcal{Y}_{1}, \mathcal{Y}_{2})-H(\mathcal{X} | \mathcal{Y}_{1})+H(\mathcal{X} | \mathcal{Y}_{1}) \\ &=[H(\mathcal{X})-H(\mathcal{X} | \mathcal{Y}_{1})]+[H(\mathcal{X} | \mathcal{Y}_{1})-H(\mathcal{X} | \mathcal{Y}_{1}, \mathcal{Y}_{2})] \\ &=I(\mathcal{X} ; \mathcal{Y}_{1})+I(\mathcal{X} ; \mathcal{Y}_{2}| \mathcal{Y}_{1}) \geq I(\mathcal{X} ; \mathcal{Y}_{1}). \end{aligned}
% \end{equation}
% \end{coro}
% Since $I(\mathcal{X};\mathcal{Y}_{1},\mathcal{Y}_{2}) \geq I(\mathcal{X};\mathcal{Y}_{1})$, we can conclude that more compromised $\mathcal{Y}$ lead to a worse situation of information leakage of $\mathcal{X}$ in favor of the attacker and our experimental results also support this conclusion. Based on the mutual information, the definition of irreversibility given in the ISO/IEC IS 24745 for cancelable biometrics under single template exposure can be reformulated as follows:

% \begin{define}
% Given a cancelable biometric transformation $f \in \mathcal{F}$ and instance $\mathcal{X}$, a protected instance $\mathcal{Y}$ is generated by $\mathcal{Y}=f(\mathcal{X};K)$, where $K$ is the parameter of $f$. If $I(\mathcal{X};\mathcal{Y})=0$, $f$ is \Stress{fully irreversible}, otherwise it is \Stress{partially irreversible}.
% \end{define}

